Accelerated Multi-Objective Alloy Discovery through Efficient Bayesian Methods: Application to the FCC Alloy Space

This study introduces BIRDSHOT, an integrated Bayesian materials discovery framework designed to efficiently explore complex compositional spaces while optimizing multiple material properties. We applied this framework to the CoCrFeNiVAl FCC high entropy alloy (HEA) system, targeting three key performance objectives: ultimate tensile strength/yield strength ratio, hardness, and strain rate sensitivity. The experimental campaign employed an integrated cyber-physical approach that combined vacuum arc melting (VAM) for alloy synthesis with advanced mechanical testing, including tensile and high-strain-rate nanoindentation testing. By incorporating batch Bayesian optimization schemes that allowed the parallel exploration of the alloy space, we completed five iterative design-make-test-learn loops, identifying a non-trivial three-objective Pareto set in a high-dimensional alloy space. Notably, this was achieved by exploring only 0.15% of the feasible design space, representing a significant acceleration in discovery rate relative to traditional methods. This work demonstrates the capability of BIRDSHOT to navigate complex, multi-objective optimization challenges and highlights its potential for broader application in accelerating materials discovery.

==> my1_packages.tex <==
%%
%%
%% DOCUMENT PACKAGES
%%
%%

%%
%% PAGE SETUP
%%


\usepackage{authblk}

\usepackage{geometry}
\geometry{left = 3em, right = 3em, top = 3em, bottom = 3em}
\geometry{includefoot}
% \geometry{nofoot}
% \geometry{showframe}
% https://ctan.org/pkg/geometry

\usepackage{tocloft}
\renewcommand\cftsecfont{\normalfont}
\renewcommand\cftsecpagefont{\normalfont}
\renewcommand{\cftsecleader}{\cftdotfill{\cftsecdotsep}}
\renewcommand\cftsecdotsep{\cftdot}
\renewcommand\cftsubsecdotsep{\cftdot}
% Table of contents with proper formatting

\usepackage{indentfirst}
% https://ctan.org/pkg/indentfirst

\usepackage{xpatch}
% https://www.ctan.org/pkg/xpatch
\xpatchcmd{\MaketitleBox}{\hrule\vskip12pt}{\vspace{-2\baselineskip}}{}{}
% Remove first horizontal rule (above abstract) + space
\xpatchcmd{\MaketitleBox}{\hrule}{}{}{}
% Remove horizontal rule after keywords

%%
%% FIGURES AND TABLES
%%

\usepackage{tabularray}
% Make good looking tables

\usepackage{makecell}
% Allows extra line within cell

\usepackage{setspace}

\usepackage{float}

\usepackage[singlelinecheck=false]{caption}
\captionsetup[table]{skip=5pt}
% https://ctan.org/pkg/caption
\captionsetup{skip = 10pt}
% Space between fig and cap
\DeclareCaptionLabelFormat{bf_parens}{(\textbf{#2})}
% Hanging setup with "(1)..." as figure numbering
\captionsetup{font={small,bf}}
\captionsetup{labelformat = bf_parens, labelsep = quad}
\captionsetup{format = hang}

% \usepackage{wrapfig}
% https://ctan.org/pkg/wrapfig
% Like word's wrapfigure

\usepackage{subcaption}
% https://www.ctan.org/pkg/subcaption
% Subcaptioning for multi-part figures (a) (b) etc.

\usepackage[table]{xcolor}
% https://ctan.org/pkg/xcolor
% Provides \cellcolor[HTML]{DDDDDD} as table background formatting

\usepackage{soul}
% https://ctan.org/pkg/soul
% Provides \cellcolor[HTML]{DDDDDD} as table background formatting

%%
%% TEXT MODIFICATIONS
%%

\usepackage[small]{titlesec}
% \titleformat{\section}
%   {\normalfont\scshape}{\thesection}{1em}{}
% \titleformat{\section}{\bfseries}{\thesection}{\MakeUppercase}
% \titleformat{\subsection}{\bfseries}{\thesubsection}

\usepackage{microtype}
% https://www.ctan.org/pkg/microtype
% Applies margin kerning to greatly improve text appearance
\microtypesetup{activate = {true, nocompatibility}}
% % activate protrusion and expansion
\microtypesetup{final}
% % enable microtype; use "draft" to disable
\microtypesetup{tracking = true}
\microtypesetup{kerning = true}
\microtypesetup{factor = 1500}
% % 1100 adds 10% to the protrusion amount (default is 1000)
\microtypesetup{stretch = 10}
\microtypesetup{shrink = 10}
% reduce defaults 20 and 20

\usepackage[hidelinks]{hyperref}
% https://ctan.org/pkg/hyperref
% Use \autoref{} instead of \ref{} for figures so that "Figure" is automatically included in the caption

\usepackage[version = 4]{mhchem}
% https://ctan.org/pkg/mhchem
% Typing formulae with multiple subscripts in a row easily
% Example syntax: accepts whole numbers and fractions
% \ce{Ni_{40.5}Ti_{20.5}Pd_{20.5}Au_{20.5}}

\usepackage[LGRgreek]{mathastext}
% Stop italicization of in line math mode
% https://ctan.org/pkg/mathastext

\usepackage{textcomp, gensymb}
% Type \degree for the degree symbol
% Explicitly importing textcomp prior to gensymb avoids warnings
% https://ctan.org/pkg/textcomp
% https://ctan.org/pkg/gensymb

%%
%% REFERENCES
%%

\usepackage[style=nature]{biblatex}
\addbibresource{supplement.bib}

% \usepackage[style = nature]{biblatex}
% \addbibresource{Bibliography.bib}
% \biblatexsetup[style = nature]

%%
%% CONVENIENCE TOOLS
%%

\usepackage{lipsum} 
% https://www.ctan.org/pkg/lipsum
% Add automatic text

\usepackage{graphicx}


==> my2_settings.tex <==
%%
%%
%% SETTINGS AND PERSONAL COMMANDS
%%
%%

% Changes to author font
\renewcommand{\Affilfont}{\mdseries \itshape \footnotesize}

\setstretch{1}

\setlength{\parskip}{0em} 
% X times font height between paragraphs

\parindent=1.5em
% 1st line paragraph spacing in each paragraph

\setlength{\columnsep}{2em}
